Retrofitting Effect Handlers onto OCaml

Effect handlers have been gathering momentum as a mechanism for modular programming with user-defined effects. Effect handlers allow for non-local control flow mechanisms such as generators, async/await, lightweight threads and coroutines to be composably expressed. We present a design and evaluate a full-fledged efficient implementation of effect handlers for OCaml, an industrial-strength multi-paradigm programming language. Our implementation strives to maintain the backwards compatibility and performance profile of existing OCaml code. Retrofitting effect handlers onto OCaml is challenging since OCaml does not currently have any non-local control flow mechanisms other than exceptions. Our implementation of effect handlers for OCaml: (i) imposes a mean 1% overhead on a comprehensive macro benchmark suite that does not use effect handlers; (ii) remains compatible with program analysis tools that inspect the stack; and (iii) is efficient for new code that makes use of effect handlers.

==> Makefile <==
paper:
	pdflatex retro-concurrency
	bibtex retro-concurrency
	pdflatex retro-concurrency
	pdflatex retro-concurrency

techrep: paper
	mkdir -p techrep
	pdflatex -output-directory techrep '\def\techreport{1}\input{retro-concurrency}'

haste:
	pdflatex retro-concurrency

retro-concurrency-sources.zip:
	mkdir -p retro-concurrency-sources
	mkdir -p retro-concurrency-sources/sandmark-notebook
	mkdir -p retro-concurrency-sources/http-benchmarks
	cp -r figures acmart.cls ACM-Reference-Format.bst retro-concurrency.bib \
		retro-concurrency.tex Makefile unicode-preamble.tex \
		retro-concurrency-sources
	cp sandmark-notebook/*.pdf retro-concurrency-sources/sandmark-notebook
	cp http-benchmarks/*.pdf retro-concurrency-sources/http-benchmarks
	zip -r retro-concurrency-sources.zip retro-concurrency-sources

graphs:
	make -C sandmark-notebook
	make -C http-benchmarks

all: techrep retro-concurrency-sources.zip

clean:
	make -C bench clean
	make -C code clean
	rm -rf *.log *.aux *.bbl *.blg *~ *.out techrep retro-concurrency-sources \
		retro-concurrency-sources.zip

